Prompt Tuning for Generative Multimodal Pretrained Models

Prompt tuning has become a new paradigm for model tuning and it has demonstrated success in natural language pretraining and even vision pretraining. In this work, we explore the transfer of prompt tuning to multimodal pretraining, with a focus on generative multimodal pretrained models, instead of contrastive ones. Specifically, we implement prompt tuning on the unified sequence-to-sequence pretrained model adaptive to both understanding and generation tasks. Experimental results demonstrate that the light-weight prompt tuning can achieve comparable performance with finetuning and surpass other light-weight tuning methods. Besides, in comparison with finetuned models, the prompt-tuned models demonstrate improved robustness against adversarial attacks. We further figure out that experimental factors, including the prompt length, prompt depth, and reparameteratization, have great impacts on the model performance, and thus we empirically provide a recommendation for the setups of prompt tuning. Despite the observed advantages, we still find some limitations in prompt tuning, and we correspondingly point out the directions for future studies. Codes are available at \url{https://github.com/OFA-Sys/OFA}

==> tables/robustness.tex <==
\begin{table*}[t]
\center
\small
\vskip 0.15in
\begin{adjustbox}{max width=1.0\textwidth}
\begin{tabular}{@{\extracolsep{\fill}}lcccccccccccccccc}
\toprule
  \multirow{2}*{Method}
  %&COCO Captions
  &\multicolumn{3}{c}{RefCOCO}
  &\multicolumn{3}{c}{RefCOCO+}
  &\multicolumn{2}{c}{RefCOCOg}
  &\multicolumn{2}{c}{SNLI-VE}
  &\multicolumn{4}{c}{COCO Captions}
  &\multicolumn{2}{c}{VQA}
 
  \\
  & val & testA & testB
  & val & testA & testB
  & val-u & test-u
  & dev & test
  & B@4 & M & C & S
  & test-dev & test-std
  \\
\midrule
    Finetune
    & 90.05 & 92.93 & 85.26
    & 85.80  & 89.87 & 79.22
    & 85.89 & 86.55
    & 90.30  & 90.20
    & 42.40 & 31.50 & 142.2 & 24.50
    & 80.40  & 80.70
    \\
    
    Prefix Tuning
    & 90.05 & 92.31 & 85.59
    & 84.54 & 89.40 & 77.77
    & 85.27 & 85.89
    & 90.04 & 90.12
    & 41.81 & 31.51 & 141.4 & 24.42
    & 78.30  & 78.53
    \\
    
    Finetune + Attacking
    & 89.68 & 92.03 & 85.23
    & 85.06 & 89.24 & 78.87
    & 85.18 & 85.50
    & 89.78 & 89.93
    & 42.28 & 31.43 & 140.8 & 24.42
    & 79.84 & 80.12
    \\
    
 
    
    Prefix Tuning + Attacking
    & 89.84 & 92.16 & 85.28
    & 84.14 & 89.08 & 77.57
    & 85.22 & 85.59
    & 89.84 & 89.98
    & 41.74 & 31.24 & 140.1 & 24.36
    & 78.01 & 78.34
    \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Experimental results on adversarial attack using large-size models.We discover that the prefix-tuning method achieves improved attack performance  on different downstream tasks.}
\label{tb:robustness}
\end{table*}
